Fast Asymptotically Optimal Kinodynamic Planning via Vectorization

Sampling-based motion planners have been shown to be effective for systems with complex kinodynamic constraints and high dimensionality. However, these algorithms struggle to achieve real-time performance, leading to recent efforts to parallelize planning. While GPU-accelerated planners have achieved significant speedups, existing approaches require specialized CUDA programming that limits accessibility and portability. We present Parallel Asymptotically Optimal Kinodynamic RRT (PAKR), a massively parallel kinodynamic planner leveraging JAX and the XLA compiler to achieve GPU acceleration through standard Python tooling. By combining our parallel planner with the AO-x meta-algorithm, we achieve asymptotic optimality through fast iterative replanning. We provide a theoretical analysis of probabilistic completeness, analyze the effects of batch size and branching factor on convergence, and demonstrate scalability to complex dynamics using the MuJoCo-XLA simulator. Experiments show competitive runtimes with state-of-the-art GPU planners and superior solution quality.

==> junk.tex <==
%Soft robots are useful for many tasks.
%In particular, there is this kind of soft robot that shows promise for some number of applciations.
%However, this robot is difficult to control and plan for due to inherent softness and strange physics.
%Analytic characterizations exist, but are limited and focus on specific aspects of interaction.
%Physics Simulation is a useful tool for control and planning, and simulators exist for vine robots,
%...but are either expensive (FEM)
%or offer a limited set of dynamics (julia sim).
%Recent advances in differentiable simulation and in particular, differentiable optimization have provided the tools necessary to lift physics sims for vine robots into efficient data-parallel impelemntations.
%This is what we provide - pytorch, etc.

\begin{comment}
\begin{enumerate}
    \item Soft/vine robots are cool, have interesting properties~\cite{hawkes2017soft,coad2019vine}.
    Modeling is a challenge~\cite{blumenschein2020design}.
    \item Why have a simulator? Key for robotics and planning, enabling accurate prediction of future behavior enabling more complex planning and estimation techniques. However, there is a sim-to-real gap, and this gap is even more pronounced when dealing with continuum bodies, friction, and contact.
    \item Accurate simulation is important, but finding appropriate parameters is tough, and fitting those parameters to real data to closely match the system is tough.
    \item We propose an end-to-end differentiable simulator for inflatable vine robots using efficient batched GPU-parallel implementations leveraging recent advances in differentiable optimization.
    Also use a different \todo{how?} model of the dynamics of the robot.
    \item Demonstrate learning some properties, show its faster \zk{is it? should be with batching}, more accurate \zk{is it? should be with modeling QP not just linearization}, show it works for modeling more closely real systems, compare against existing simulation frameworks.
    \item Open source implementation using PyTorch~\cite{paszke2019pytorch} available\footnote{\url{https://github.com/CoMMALab/DiffVineSimPy}}.
\end{enumerate}
\end{comment}


% Soft robot simulation inherently difficult, contact and deformable objects require expensive simulation to do accurately
% FEM methods are popular for accurate simulation, and for vine robots have been used to model their growth, buckling, and even sheath extension
% Need faster than real time simulation for effective planning / control
% Video game simulators and dynamic models have been used
% These however have issues with precision, and are difficult to integrate into end-to-end optimization - single time step is possible


%What are vine robots? Explain some basics.
%Vine robot modeling and planning - heuristic/analytic models used in works like~\cite{greer2020robust}. 
%\zk{analytic~\cite{blumenschein2021geometric,selvaggio2020obstacle,greer2020robust}}
%\lhb{The other modeling works that exist are typically concerned with the growth \cite{blumenschein2017modeling,haggerty2019characterizing}, though there have been a few other works looking at specific events in buckling similar to \cite{greer2020robust}, such as some paarts of \cite{haggerty2019characterizing} and buckling during retraction \cite{coad2020retraction} and buckling during unsuspended growth \cite{mcfarland2023collapse}}
%Probably need to throw in discussion of constant pressure = constant stiffness assumption (? not 100\% sure on the actual modeling here).
%\lhb{The paper that is the basis of this assumption is \cite{comer1963deflections}, but Sicheng's recent paper~\cite{wang2024anisotropic} has a breakdown of how this model can be extended beyond that simplifying assumption}

    
%Existing simulators for vine robots are either FEM~\cite{du2023finite} using frameworks like %SOFA~\cite{faure2012sofa}.
%FEM simulators for vine robots.
%Steerable one~\cite{li2021bioinspired}.
%MAMMOBot~\cite{vartholomeos2024lumped}, 
%also one built on top of SOFA and models sheath~\cite{wu2023towards}.
%Maximal coordinates - series of rigid bodies simulators.
%Unity~\cite{el2018development}.
%Constant-size impulse velocity Lagrange multiplier~\cite{jitosho2021dynamics}, 
%Issues with speed with FEM, precision with analytic due to unmodeled effects like friction and buckling, Julia sim is only slightly faster than real time.

%Diffsim even cooler and emerging as a powerful tool in robotics~\cite{collins2021review} for doing identification, neural models, batching, etc. Allows for propagation of gradients through the simulation, and has been used to great success in reinforcement learning, optimal control, and parameter fitting for complex dynamics in a scene.
% works for rigid body dynamics~\cite{heiden2021neuralsim, howell2022dojo}.
%\zk{Note that DOJO~\cite{howell2022dojo} enables simulation of stiff contacts for rigid bodies}.

%Really cool potential applications in planning and manipulation~\cite{toussaint2018differentiable}.
%Could be used for inverse problem formulation - what contacts do we want to make, e.g.,~\cite{coevoet2017optimization}.


%Diffsim for soft robotics.
% Diffsim has been used in soft robotics before, e.g., Chainqueen~\cite{hu2019chainqueen}, but only applied to deformables, not everting pneumatic vines, also in the underwater case~\cite{du2021underwater}.
 
%Learned models have been used as differentiable physical models~\cite{bern2020soft}.
%Diffsim used in learning and optimizing soft robot design~\cite{spielberg2019learning} - could be used here as well, as modeling is essential for rapid design, not just optimizing design~\cite{mengaldo2022concise}.

%Diffsim for parameter identification.
%We focus on learning parameters using DiffSim as an enabling feature, e.g.,~\cite{le2021differentiable,jatavallabhula2021gradsim} - learning parameters~\cite{lee2023robot} is essential.

We also wish to investigate issues with high stiffness in high pressure regimes for buckling behavior.

There are many potential avenues of future research with end-to-end differentiability, such as MPC/MPPI, inverse modeling to find robot designs that achieve specific behavior, reinforcement learning, optimizing robot designs, and more.

\begin{enumerate}
    \item Introduced differentiable vine robot simulator implemented in pytorch, open source, look at the code.
    \item Demonstrated effectiveness, showed how it could be used for doing parameter matching of real robot data.
    \item What doors does this open up? Batch rollouts buy planning power, MPC/MPPI, possibly differentiable MPC~\cite{amos2018differentiable}? Physical parameter identification for advanced physics? Buckling? Neural physics models for contacts, etc? Can this be integrated in bigger end-to-end neural models? Inverse modeling: planning sequences of contacts, manipulation with vine robots?
    \item Stiffness and issues with differentiable simulation gradients~\cite{suh2022differentiable}.
    \item Contact is hard in diffsim~\cite{le2023single}.due to sparse gradients, methods that circumvent this exist, e.g.,~\cite{antonova2023rethinking}.
    \item Future work: speed, additional physical parameters, moving to the 3D case, adding additional modes of actuation (pinch points, welds, tension, etc.).
\end{enumerate}
